QuestGen: Effectiveness of Question Generation Methods for Fact-Checking Applications

Verifying fact-checking claims poses a significant challenge, even for humans. Recent approaches have demonstrated that decomposing claims into relevant questions to gather evidence enhances the efficiency of the fact-checking process. In this paper, we provide empirical evidence showing that this question decomposition can be effectively automated. We demonstrate that smaller generative models, fine-tuned for the question generation task using data augmentation from various datasets, outperform large language models by up to 8%. Surprisingly, in some cases, the evidence retrieved using machine-generated questions proves to be significantly more effective for fact-checking than that obtained from human-written questions. We also perform manual evaluation of the decomposed questions to assess the quality of the questions generated.

==> cikm24-short-pc.tex <==
Amin Abolghasemi	Leiden University
	Muhammad Abulaish	South Asian University
	Muhammad Abdullah Adnan	University of California San Diego
	Rahul Agrawal	Sharechat
	Dirk Ahlers	NTNU - Norwegian University of Science and Technology
	Wasi Ahmad	Amazon Web Services
	Qingyao Ai	Tsinghua University
	Monika Akbar	University of Texas at El Paso
	Navot Akiva	CS Dept, Bar Ilan University
	Khalil Al Hussaeni	RIT-Dubai
	Mehwish Alam	Telecom paris
	Dyaa Albakour	Signal AI
	Hamed Alhoori	Northern Illinois University
	James Allan	University of Massachusetts Amherst
	May Altulyan	PSAU
	Ikram Amous	MIRACL
	Aijun An	York University
	David Anastasiu	Santa Clara University
	Vito Walter Anelli	Politecnico di Bari
	Sarah Anjum	Santa Clara University
	Kemafor Anyanwu	North Carolina State University
	Hassina Aouidad Aliane	CERIST
	Negar Arabzadeh	University of Waterloo
	Samin Aref	University of Toronto
	Diego Arroyuelo	Department of Computer Science, Escuela de Ingeniería, Pontificia Universidad Católica de Chile
	Sunil Aryal	Deakin University
	Javed Aslam	Northeastern University
	Giuseppe Attardi	Università di Pisa
	Maurizio Atzori	University of Cagliari
	Tanja Auge	University of Regensburg
	Sandeep Avula	Amazon
	Berkay Aydin	Georgia State University
	Ebrahim Bagheri	Ryerson University
	Ashraf Bah Rabiou	University of Delaware
	Xiao Bai	Yahoo Research
	Wolf-Tilo Balke	Institut für Informationssysteme, TU Braunschweig
	Zhifeng Bao	RMIT Center of Information Discovery and Data Analytics
	Ramesh Baral	Florida International University
	Oren Barkan	TAU
	Roberto Basili	Dept. of Enterprise Engineering - Univ. of Roma Tor Vergata
	Marcos Bedo	UFF
	Amin Beheshti	Macquarie University
	Khalid Belhajjame	PSL, Université Paris-Dauphine, LAMSADE
	Nicholas Belkin	Rutgers University
	Patrice Bellot	Aix-Marseille Université - CNRS (LIS)
	Andras A. Benczur	Institute for Computer Science and Control, Hungarian Academy of Sciences
	Gerd Berget	Oslo Metropolitan University
	Rafael Berlanga	Universitat Jaume I
	Anurag Bhardwaj	eBay Research Labs
	Kaustav Bhattacharjee	New Jersey Institute of Technology
	Sanjukta Bhowmick	University of North Texas
	Keping Bi	Institute of Computing Technology, Chinese Academy of Sciences
	Xin Bi	Northeastern University
	Devis Bianchini	University of Brescia
	Christian Bizer	University of Mannheim
	Veronika Bogina	Tel Aviv University
	Ludovico Boratto	University of Cagliari
	José Borbinha	Universidade de Lisboa
	Mohamed Reda Bouadjenek	Deakin University
	Larbi Boubchir	University of Paris 8
	Eric Boxer	University of Southern California
	Vanessa Braganholo	Universidade Federal Fluminense (UFF)
	Pavel Braslavski	Ural Federal University
	Adrian M.P. Brasoveanu	MODUL Technology GmbH
	Ali Braytee	University of Technology, Sydney
	Timo Breuer	TH Köln (University of Applied Sciences)
	Pierangela Bruno	University of Calabria
	Francesco Buccafurri	Università Mediterranea di Reggio Calabria
	Alexander Buchholz	Amazon
	Guntur Budi Herwanto	Universitas Gadjah Mada
	Peng Cai	East China Normal University
	Zekun Cai	The University of Tokyo
	Sylvie Calabretto	LIRIS
	Jean-Paul Calbimonte	University of Applied Sciences and Arts Western Switzerland HES-SO
	Ricardo Campos	University of Beira Interior; INESC TEC; Ci2 Smart Cities Research Center (Polytechnic Institute of Tomar)
	Fazli Can	Bilkent University
	K. Selcuk Candan	Arizona State University
	Longbing Cao	Faculty of IT, University of Technology Sydney
	Yuanjiang Cao	Macquarie University
	Cinzia Cappiello	Politecnico di Milano
	Alycia Carey	University of Arkansas
	Yukuo Cen	Tsinghua University
	Aniket Chakrabarti	Amazon
	Anirban Chakraborty	University of Wolverhampton
	Harry Kai-Ho Chan	University of Sheffield
	Zhangming Chan	Alibaba Group
	Lijun Chang	The University of Sydney
	Shubham Chatterjee	University of Edinburgh
	Animesh Chaturvedi	Indian Institute of Information Technology Dharwad
	Despoina Chatzakou	Information Technologies Institute, Centre for Research and Technology Hellas
	Catherine Chavula	University of Strathclyde
	Bo Chen	Huawei Noah's Ark Lab
	Bowei Chen	University of Glasgow
	Chen Chen	University of Wollongong
	Chung-Chi Chen	National Institute of Advanced Industrial Science and Technology
	Emily Chen	University of Southern California
	Feng Chen	UT Dallas
	Hao Chen	Beihang University
	Hsin-Hsi Chen	National Taiwan University
	Jiawei Chen	Zhejiang University
	Jin Chen	
	Lu Chen	Swinburne University of Technology
	Ruey-Cheng Chen	Canva
	Wei Chen	Soochow University
	Xiang Chen	ZheJiang University
	Yankai Chen	The Chinese University of Hong Kong
	Yi Chen	New Jersey Institute of Technology
	Yinlin Chen	Virginia Tech
	Zhiqian Chen	Mississippi State University
	Ziheng Chen	Stony Brook University
	Gong Cheng	Nanjing University
	Peng Cheng	East China Normal University
	Xuntao Cheng	Alibaba Group
	Yihang Cheng	BOSS Zhipin
	Zhiyong Cheng	Shandong Artificial Intelligence Institute
	Fei Chiang	McMaster University
	Adrian-Gabriel Chifu	Aix Marseille Univ, Université de Toulon, CNRS, LIS
	Jin Yao Chin	Nanyang Technological University
	Rada Chirkova	North Carolina State University
	Theodoros Chondrogiannis	University of Konstanz
	Philipp Christmann	Max Planck Institute for Informatics, Saarland Informatics Campus
	Lingyang Chu	McMaster University
	Lin Chung-Yi	National Taiwan University
	Malcolm Clark	The University of the Highlands & Islands
	Luca Colomba	Politecnico di Torino
	Simona Colucci	Politecnico di Bari
	Cristian Consonni	Eurecat - Centre Tecnològic de Catalunya
	Fabio Cozman	University of São Paulo
	Gregory Crane	Tufts University
	Fabio Crestani	Università della Svizzera Italiana (USI)
	Lizhen Cui	School of Computer Science and Technology, Shandong University, Jinan, P. R. China
	Shiyao Cui	
	Bertrand Cuissart	GREYC
	Alfredo Cuzzocrea	University of Calabria
	Altigran da Silva	Universidade Federal do Amazonas
	Hua Dai	Nanjing University Of Posts and Telecommunications
	Ariyam Das	Google
	Anwitaman Datta	Nanyang Technological University
	Suchana Datta	University College Dublin
	Kenny Davila	DePaul University
	Brian Davison	Lehigh University
	Ernesto William De Luca	Georg-Eckert-Institute – Leibniz-Institute for international Textbook Research
	Edleno Silva De Moura	Universidade Federal do Amazonas
	Toon De Pessemier	Ghent University
	Victoria Degeler	University of Amsterdam
	Francesco Del Buono	University of Modena and Reggio Emilia
	Yashar Deldjoo	Polytechnic University of Bari
	Liwei Deng	University of Electronic Science and Technology of China
	Danilo Dessì	GESIS – Leibniz Institute for the Social Sciences
	Emanuele Di Buccio	University of Padua
	Giorgio Maria Di Nunzio	University of Padua
	Djellel Difallah	NYU
	Jingtao Ding	Tsinghua University, Beijing, P.R.China
	Yue Ding	Shanghai Jiao Tong University
	Nemanja Djuric	Aurora Innovation, Inc.
	Taoufiq Dkaki	IRIT, Intitut de Recherche en Informatique de Toulouse
	Vlastislav Dohnal	Faculty of Informatics, Masaryk University
	Peter Dolog	Aalborg University
	Hai Dong	RMIT University
	Yushun Dong	University of Virginia
	Carina Dorneles	UFSC
	Zhicheng Dou	Renmin University of China
	Mauro Dragoni	Fondazione Bruno Kessler - FBK-IRST
	Eduard Dragut	Temple University
	George Drosatos	Athena Research Center
	Jing Du	Macquarie University
	Wei-Wei Du	National Yang Ming Chiao Tung University
	Yuntao Du	Purdue University
	Stefania Dumbrava	ENSIIE Paris-Evry, France
	Sourav Dutta	Huawei Research
	Shusaku Egami	National Institute of Advanced Industrial Science and Technology
	Koji Eguchi	Hiroshima University
	Vinu Ellampallil Venugopal	International Institute of Information Technology, Bangalore
	Tamer Elsayed	Qatar University
	Faezeh Ensan	Toronto Metropolitan University
	Mahdi Esmailoghli	Technische Universität Berlin
	Anjie Fang	Amazon.com
	Liri Fang	University of Illinois at Urbana-Champaign
	Yi Fang	Santa Clara University
	Yixiang Fang	The Chinese University of Hong Kong, Shenzhen
	Hossein Fani	University of Windsor
	Hao Fei	National University of Singapore
	Fuli Feng	University of Science and Technology of China
	Xiaoyue Feng	Jilin University
	Yue Feng	UCL
	Yunhe Feng	University of North Texas
	Amine Ferdjaoui	Université Paris Cité
	Marcos Fernández Pichel	Universidade de Santiago de Compostela
	Peter M. Fischer	Universität Augsburg, Institut für Informatik
	Sebastien Fournier	Université d'aix-Marseille, CNRS
	Reva Freedman	Northern Illinois University
	Christoph M. Friedrich	University of Applied Sciences and Arts Dortmund; Department of Computer Science
	Ingo Frommholz	University of Wolverhampton
	Cong Fu	Texas A&M University
	Yanjie Fu	Arizona State University
	Ken Fukuda	National Institute of Advanced Industrial Science and Technology (AIST)
	Benjamin C. M. Fung	McGill University
	Maria Gaede	Humboldt-Universität zu Berlin, Berlin School of Library and Information Science
	Renata Galante	UFRGS
	Sebastien Gambs	Université du Québec à Montréal
	Debasis Ganguly	University of Glasgow
	Chen Gao	Tsinghua University
	Wanfu Gao	Jilin University
	Weibo Gao	University of Science and Technology of China
	Xiaofeng Gao	Shanghai Jiao Tong University
	Yunjun Gao	Zhejiang University
	Muskan Garg	Mayo Clinic
	Ritik Garg	Extramarks Education Pvt Ltd
	Dario Garigliotti	University of Bergen
	Ekaterina Garmash	Spotify
	Paolo Garza	Politecnico di Torino
	Kripabandhu Ghosh	Indian Institute of Science Education and Research (IISER) Kolkata, India
	Philippe Giabbanelli	Miami University
	Joan Giner Miguelez	Universitat Oberta de Catalunya
	Daniela Godoy	ISISTAN Research Institute (UNCPBA-CONICET)
	Alberto González Martínez	University Of Hawaii at Manoa
	Anastasios Gounaris	Aristotle University of Thessaloniki
	Michael Granitzer	University of Passau
	David Gross-Amblard	Univ Rennes - CNRS - IRISA
	Francesco Guerra	Università di Modena e Reggio Emilia
	Giovanna Guerrini	DIBRIS- University of Genova
	Jie Gui	University of Michigan
	Shurui Gui	Texas A&M University
	Riccardo Guidotti	University of Pisa
	Giacomo Guiduzzi	University of Modena and Reggio Emilia
	Francesco Gullo	University of L'Aquila
	Guimu Guo	Rowan University
	Stephen Guo	Indeed
	Ting Guo	University of Technology Sydney
	Wei Guo	Huawei Singapore Research Center
	Wentian Guo	Meta Inc.
	Xingzhi Guo	Stony Brook University
	Dhruv Gupta	Norwegian University of Science and Technology
	Cathal Gurrin	Dublin City University
	Ido Guy	Facebook
	Zhen Hai	Institute for Infocomm Research, A*STAR, Singapore
	Sherzod Hakimov	University of Potsdam
	Nur Al Hasan Haldar	The University of Western Australia
	Jinyoung Han	Sungkyunkwan University
	Shuchu Han	StellarCyber.ai
	Shuguang Han	Google
	Xiaolin Han	Northwestern Polytechnical University
	Junheng Hao	University of California, Los Angeles
	Fatima Haouari	Qatar University
	Ehsan Ul Haq	The Hong Kong University of Science and Technology
	Sven Hartmann	Clausthal University of Technology
	Maram Hasanain	Qatar University
	Guoxiu He	East China Normal University
	Jiayuan He	RMIT University
	Jiyin He	Signal AI
	Kshiteesh Hegde	Western Digital
	Danula Hettiachchi	RMIT University
	Xu Hongbo	Institute of Information Engineering， CAS
	Sayed Hoseini	Hochschule Niederrhein
	Yupeng Hou	University of California, San Diego
	Binbin Hu	Ant Group
	Jun Hu	School of Computing, National University of Singapore
	Wei Hu	Nanjing University
	Xuanming Hu	Arizona State University
	Xuming Hu	
	Yifan Hu	Yahoo!
	Wency Hua	Hong Kong Polytechnic University
	Chao Huang	University of Notre Dame
	Chengkai Huang	The University of New South Wales
	Jen-Wei Huang	National Cheng Kung University
	Jiantao Huang	National Taiwan University, Taiwan, ROC
	Jimmy Huang	York University
	Junzhou Huang	The University of Texas at Arlington
	Keke Huang	National University of Singapore
	Weiming Huang	Nanyang Technological University
	Zhuo Huang	Nanjing University of Science and Technology
	Kai Hui	Google
	Dongmin Hyun	Yahoo
	Dmitry Ilvovsky	National Research University Higher School of Economics
	Oana Inel	University of Zurich
	Amir Ingber	Pinecone
	Bogdan Ionescu	Politehnica University of Bucharest
	Radu Tudor Ionescu	University of Bucharest, Faculty of Mathematics and Computer Science
	Roshni Iyer	University of California, Los Angeles
	Amit Kumar Jaiswal	University of Surrey
	Adam Jatowt	University of Innsbruck
	Olivier Jeunen	ShareChat UK
	Shiyu Ji	UCSB
	Yiling Jia	Google Research
	Zhen Jia	School of Computing and Artificial Intelligence, Southwest Jiaotong University
	Lu Jiang	Northeast Normal University
	Renhe Jiang	The University of Tokyo
	Zhimeng Jiang	Texas A&M University
	Zhuoren Jiang	Zhejiang University
	Beihong Jin	Institute of Software, Chinese Academy of Sciences
	Gareth Jones	Dublin City University
	Shawn Jones	Los Alamos National Laboratory
	Joemon Jose	University of Glasgow
	Ozan Kahramanogullari	Free Unversity of Bozen-Bolzano, Faculty of Computer Science
	Anup Kalia	IBM
	Jaap Kamps	University of Amsterdam
	Verena Kantere	University of Ottawa
	Pinar Karagoz	Middle East Technical University (METU)
	Pranav Kasela	University of Milano-Bicocca
	Makoto P. Kato	University of Tsukuba
	Mayank Kejriwal	Information Sciences Institute
	Roman Kern	Know-Center GmbH
	Arijit Khan	Aalborg University
	Maleq Khan	Texas A&M Univeristy-Kingsville
	Evgeny Kharlamov	Bosch
	Aparup Khatua	University of Michigan
	Maria Khodorchenko	ITMO University
	Yubin Kim	Etsy, Inc.
	Tracy Holloway King	Adobe
	Alexander Kirillovich	ex. HSE University
	Praveen Kolli	DoorDash Inc
	Valia Kordoni	
	Yuta Koreeda	Hitachi, Ltd.
	Yehuda Koren	Google
	Manolis Koubarakis	National and Kapodistrian University of Athens
	Adit Krishnan	IIT Madras
	Udo Kruschwitz	University of Regensburg
	Oren Kurland	Technion
	Saar Kuzi	Amazon
	Wai Lam	The Chinese University of Hong Kong
	Renaud Lambiotte	University of Oxford
	Rabindra Lamsal	The University of Melbourne
	Geon Lee	Korea Advanced Institute of Science and Technology
	Grace E. Lee	Thomson Reuters
	Kyong-Ho Lee	Yonsei University
	Seokki Lee	University of Cincinnati
	Teerapong Leelanupab	University of Queensland
	Chen Lei	HeFei University of Technology
	Jochen L. Leidner	Coburg University of Applied Sciences / University of Sheffield / KnowledgeSpaces
	Bo Li	Peking University
	Bohan Li	Nanjing university of aeronautics and astronautics
	Chao Li	Beijing Jiaotong University
	Cheng Li	Google
	Chenliang Li	Wuhan University
	Huan Li	Zhejiang University
	Hui Li	Xidian University
	Jiayang Li	University of Electronic Science and Technology of China
	Ke Li	University of Exeter
	Lei Li	The Hong Kong University of Science and Technology (Guangzhou)
	Mingzhe Li	Peking University
	Ruizhe Li	University of Aberdeen
	Shuai Li	Cambridge University
	Wei Li	Jiangnan university
	Ximing Li	Jilin university
	Xiner Li	Texas A&M University
	Xinhang Li	Tsinghua University
	Xinshu Li	University of New South Wales, Australia
	Yanzeng Li	Institute of Information Engineering, Chinese Academy of Sciences
	Yingjie Li	JPMorgan Chase
	Yuan Li	North China University of Technology
	Zhenhui Li	Yunqi Academy of Engineering
	Zhi Li	University of Science and Technology of China
	Zihan Li	University of Massachusetts Boston
	Panagiotis Liakos	NKUA
	Defu Lian	University of Science and Technology of China
	Xiang Lian	Kent State University
	Hongwei Liang	Microsoft
	Jz Liao	National University of Defense Technology
	Lizi Liao	Singapore Management University
	Ningyi Liao	Nanyang Technological University
	Alexander Libov	Amazon
	Sergio Lifschitz	PUC-Rio
	Kwan Hui Lim	Singapore University of Technology and Design
	Hongfei Lin	Dalian University Of Technology
	Qika Lin	Xi'an Jiaotong University
	Wenqing Lin	Tencent
	Anna Sofia Lippolis	CNR ISTC
	Bang Liu	University of Montreal
	Dugang Liu	Shenzhen University
	Fei Liu	Hefei University of Technology
	Fenglin Liu	University of Oxford
	Guanfeng Liu	Macquarie University
	Haiming Liu	School of Electronics and Computer Science, University of Southampton
	Hanpeng Liu	Univeristy of Southern California
	Hongtao Liu	Du Xiaoman Financial
	Jingjing Liu	MD Anderson Cancer Center
	Jiqun Liu	University of Oklahoma
	Kunpeng Liu	Portland State University
	Lei Liu	York University
	Qi Liu	University of Science and Technology of China
	Shuncheng Liu	University of Electronic Science and Technology of China
	Tingting Liu	National Institute on Drug Abuse, National Institutes of Health
	Weiming Liu	Zhejiang University
	Xiaoguang Liu	Nankai University
	Ye Liu	Salesforce
	Yiqun Liu	Tsinghua University
	Yu-An Liu	Institute of Computing Technology, Chinese Academy of Sciences
	Yue Liu	NUDT
	Zitao Liu	Guangdong Institute of Smart Education, Jinan University
	Hamed Loghmani	University of Windsor
	Ramon Lopes	Petrobras
	Yin Lou	Ant Group
	Natalia Loukachevitch	Research Computing Center of Moscow State University
	Chang-Tien Lu	VT
	Guangquan Lu	Sun Yat-sen University
	Wei Lu	wuhan university
	Cheng Luo	Tsinghua University
	Jiyun Luo	Pinterest
	Junyu Luo	Pennstate University
	Xiao Luo	Department of Computer Science, UCLA
	Youzhi Luo	Amazon
	Fuyuan Lyu	McGill University
	Hanjia Lyu	University of Rochester
	Chen Ma	City University of Hong Kong
	Chenhao Ma	The Chinese University of Hong Kong, Shenzhen
	Hehuan Ma	University of Texas at Arlington
	Junbo Ma	Guangxi Normal University
	Xiaogang Ma	University of Idaho
	Sofian Maabout	LaBRI. University of Bordeaux
	Khushhall Chandra Mahajan	Meta Inc.
	Daniele Malitesta	Université Paris-Saclay
	Antonio Mallia	New York University
	Hiroshi Mamitsuka	Kyoto University / Aalto University
	Thomas Mandl	University of Hildesheim
	Paolo Manghi	ISTI-CNR
	Behrooz Mansouri	University of Southern Maine
	Jiali Mao	East China Normal University
	Jiaxin Mao	Renmin University of China
	Stefano Marchesin	University of Padova
	Mirko Marras	University of Cagliari
	Bruno Martins	IST and INESC-ID - Instituto Superior Técnico, University of Lisbon
	Flavio Martins	INESC-ID, Instituto Superior Técnico, Universidade de Lisboa
	Luis Martínez	University of Jaén
	Maarten Marx	University of Amsterdam
	Afra Mashhadi	UW
	Alexander Matiushkin	eBay
	Uwe Mayer	eBay Data Labs
	John P. McCrae	National University of Ireland, Galway
	Ida Mele	IASI-CNR
	Gabor Melli	LegalOn Technologies
	Marcelo Mendoza	Pontificia Universidad Católica de Chile
	Chuan Meng	University of Amsterdam
	Hao Miao	Aalborg University
	Helena Mihaljevic	University of Applied Sciences Berlin
	Zoltan Miklos	University of Rennes 1
	Cheng Mingyue	
	Nguyen Minh-Tien	UTEHY
	Rishabh Misra	Twitter, Inc
	Paolo Missier	Newcastle University
	Arvin Moazemi	Bocconi University
	Ashwin Shreyas Mohan Rao	Information Sciences Institute - University of Southern California
	Ali Montazeralghaem	university of massachusetts amherst
	Sebastian Moreno	Universidad Adolfo Ibañez
	Yasufumi Moriya	Dublin City University
	Yashar Moshfeghi	University of Strathclyde
	Ahmed Mourad	Apeiros Lab
	Philippe Mulhem	LIG-CNRS
	Cristina Ioana Muntean	ISTI CNR
	Elham Naghizade	RMIT University
	Mirco Nanni	KDD-Lab ISTI-CNR Pisa
	Franco Maria Nardini	ISTI-CNR
	Tal Neiman	Amazon
	Hoang Long Nguyen	Meharry Medical College
	Van-Hau Nguyen	Faculty of Information Technology, Hung Yen University of Technology and Education
	Liqiang Nie	Harbin Institute of Technology (Shenzhen)
	Ping Nie	peking university
	Andriy Nikolov	AstraZeneca
	Bo Ning	Dalian Maritime University
	Xia Ning	The Ohio State University
	Zhiyuan Ning	Computer Network Information Center, Chinese Academy of Sciences. University of Chinese Academy of Sciences.
	Annisa Maulida Ningtyas	Technische Universität Wien
	Di Niu	University of Alberta
	Shuzi Niu	Institute of Software, Chinese Academy of Sciences
	Xi Sunshine Niu	UNC Charlotte
	Alexandros Ntoulas	National and Kapodistrian University of Athens
	Sérgio Nunes	INESC TEC and Faculty of Engineering, University of Porto
	Neil O'Hare	Yahoo Research
	Theresa Omodunbi	Obafemi Awolowo University, Ile-Ife, Nigeria
	Vincent Oria	NJIT
	Aomar Osmani	LIPN-UMR CNRS 7030 , université Paris 13
	David Otero	University of A Coruña
	Iadh Ounis	University of Glasgow
	Jiaul Paik	IIT Kharagpur
	Balaji Palanisamy	University of Pittsburgh
	Shubham Singh Paliwal	TCS
	George Pallis	University of Cyprus
	Le Pan	University of New South Wales
	Yue Pang	Peking University
	George Papadakis	National Technical University of Athens
	Panagiotis Papadakos	ERCIM
	Primal Pappachan	Pennsylvania State University
	Eunju Park	Sungkyunkwan
	Ioannis Partalas	Expedia
	Bibek Paudel	Stanford University
	Pavel Pecina	Charles University
	Hao Peng	Beihang University
	Xueping Peng	University of Technology, Sydney
	Maria Soledad Pera	TUDelft
	Raffaele Perego	ISTI-CNR
	Denilson Pereira	Universidade Federal de Lavras
	Sujan Perera	IBM Watson
	Ladislav Peska	Faculty of Mathematics and Physics, Charles University, Prague, Czechia
	Casper Petersen	Sampension A/S
	Lighton Phiri	University of Zambia
	Francesco Pierri	Politecnico di Milano
	Joao Pimentel	UFF
	Fabio Pinelli	IMT Lucca
	Rajesh Piryani	IRIT - Equipe MELODI Universite Paul Sabatier
	Manolis Pitsikalis	NCSR Demokritos
	Vassilis Plachouras	Facebook
	Barbara Poblete	University of Chile
	Marco Polignano	Università degli Studi di Bari Aldo Moro
	Amey Porobo Dharwadker	Meta
	Utkarsh Porwal	University at Buffalo-SUNY
	Anastasiia Potiagalova	Dublin City University
	Jędrzej Potoniec	Poznan University of Technology
	Faryaneh Poursardar	Old Dominion University
	Romila Pradhan	Purdue University
	Erasmo Purificato	Otto von Guericke University Magdeburg
	Ji Qi	Tsinghua University
	Jianzhong Qi	The University of Melbourne
	Buyue Qian	Xi'an Jiaotong University
	Kun Qian	Columbia University
	Weizhu Qian	Aalborg University
	Jipeng Qiang	Yangzhou University
	Zhou Qin	Amazon
	Hefei Qiu	UMass Boston
	Davood Rafiei	University of Alberta
	Ashiqur Rahman	Northern Illinois University
	Fiana Raiber	Yahoo Research
	Weixiong Rao	Tongji University
	Lida Rashidi	RMIT University
	Chotirat Ratanamahatana	Chulalongkorn University
	Sagnik Ray Choudhury	NBME
	Gábor Recski	TU Wien
	Marek Reformat	University of Alberta
	Georg Rehm	DFKI
	Jiayang Ren	The University of British Columbia
	Pengjie Ren	Shandong University
	Weijeying Ren	The Pennsylvania State University
	Zhaochun Ren	Leiden University
	Anja Reusch	Technische Universität Dresden
	Thomas Risse	University Frankfurt, University Library J. C. Senckenberg
	Carlos R. Rivero	Rochester Institute of Technology
	Giuseppe Rizzo	LINKS Foundation
	Adam Roegiest	Zuva
	Haggai Roitman	eBay Research
	Federica Rollo	University of Modena and Reggio Emilia
	Giulio Rossetti	KDD Lab ISTI-CNR
	Dwaipayan Roy	Indian Institute of Science Education and Research, Kolkata
	Koustav Rudra	Indian Institute of Technology Kharagpur
	Karankumar Sabhnani	84.51°
	Fahad Saeed	Florida International University (FIU)
	Harshita Sahijwani	Emory University
	Deepak Saini	Microsoft Research
	Janete Saldanha Bach	GESIS – Leibniz Institute for the Social Sciences
	Camilla Sancricca	Politecnico di Milano
	Eric Sanjuan	Laboratoire Informatique d'Avignon- Université d'Avignon
	Maria Luisa Sapino	Universita' di Torino
	Shawon Sarkar	University of Washington
	Sougata Sarkar	Master's Student
	Nishanth Sastry	King's College London
	Markus Schedl	Johannes Kepler University Linz (JKU)
	Ralf Schenkel	Trier University
	Moritz Schubotz	FIZ Karlsruhe – Leibniz Institute for Information Infrastructure
	Martin Schäler	University of Salzburg
	Florence Sedes	I.R.I.T. Univ. Toulouse III Paul Sabatier
	Venkata Devesh Reddy Seethi	Northern Illinois University
	Christophe Servan	Qwant Research
	Shirin Seyedsalehi	Toronto Metropolitan University
	Alyssa Sha	Australian National University
	Abdul Rahman Shaikh	Northern Illinois University
	Monika Sharma	TCS Research
	Jialie Shen	City, University of London UK
	Jiawei Sheng	Institute of Information Engineering, Chinese Academy of Sciences
	Qiang Sheng	Chinese Academy of Sciences
	Boshen Shi	Institute of Computing Technology
	Min Shi	Hunan University of Science and Technology
	Yue Shi	Facebook
	Samiha Shimmi	Northern Illinois University
	Roee Shraga	Worcester Polytechnic Institute
	Zihua Si	Renmin University of China
	A.B. Siddique	University of Kentucky
	Satyaki Sikdar	Indiana University
	Fabrizio Silvestri	University of Rome
	Shruti Singh	IIT Gandhinagar
	Amit Somech	Bar-Ilan University
	Qi Song	University of Science and Technology of China
	Xuemeng Song	Shandong University
	Hugo Sousa	INESC TEC
	Marc Spaniol	Université de Caen Normandie
	Giancarlo Sperlì	University of Naples
	Francesca Spezzano	Boise State University
	Kavitha Srinivas	IBM
	Kostas Stefanidis	Tampere University
	Nikolaos Stylianou	Information Technologies Institute, Centre for Research and Technology Hellas
	Kazunari Sugiyama	Osaka Seikei University
	Yasunobu Sumikawa	Takushoku University
	Guohao Sun	Donghua University
	Peijie Sun	Hefei University of Technology, School of Computer and Information
	Tao Sun	Bytedance
	Weiwei Sun	Shandong University
	Zhu Sun	Agency for Science, Technology and Research (A*STAR)
	Reem Suwaileh	Qatar University
	Moysis Symeonides	University of Cyprus
	Keishi Tajima	Kyoto University
	Bo Tang	Southern University of Science and Technology
	Jintao Tang	School of Computer, National University of Defense Technology
	Ruixiang Tang	Rice University
	Xing Tang	FiT,Tencent
	Junichi Tatemura	Google
	Shirish Tatikonda	Walmart Labs
	Nikolaj Tatti	University of Helsinki
	Leila Tavakoli	RMIT University
	Carla Teixeira Lopes	University of Porto
	Tommaso Teofili	Roma Tre University
	Paul Thomas	Microsoft
	Camilo Thorne	Elsevier
	Gabriele Tolomei	Sapienza University of Rome
	Antonela Tommasel	ISISTAN Research Institute, CONICET-UNCPBA
	Ito Tomoki	The University of Tokyo
	Nicola Tonellotto	University of Pisa
	Hanghang Tong	University of Illinois at Urbana-Champaign
	Shiwei Tong	University of Science and Technology of China
	Yongxin Tong	Beihang University
	Cagri Toraman	Aselsan Research Center
	Ali Tourani	Interdisciplinary Center for Security Reliability, and Trust (SnT), University of Luxembourg
	Demetris Trihinas	University of Nicosia
	Andrew Trotman	University of Otago
	Christos Tryfonopoulos	University of Peloponnese
	Manos Tsagkias	Apple
	Vincent Tseng	National Chiao Tung University
	Ilya Tyagin	University of Delaware
	Takanori Ugai	Fujitsu Limited
	Md Zia Ullah	Edinburgh Napier University
	Kazutoshi Umemoto	The University of Tokyo
	Prajna Upadhyay	BITS Pilani Hyderabad Campus
	Julián Urbano	Delft University of Technology
	Hossein Vahabi	UC Berkeley
	Siva Likitha Valluru	University of South Carolina
	Christophe Van Gysel	Apple Inc.
	Francielle Vargas	University of São Paulo
	Pedro Vaz-de-Melo	UFMG
	Manisha Verma	Amazon
	Stefanos Vrochidis	Information Technologies Institute
	Shaohua Wan	School of Information and Safety Engineering, Zhongnan University of Economics and Law
	Sheng Wan	Nanjing University of Science and Technology
	Beilun Wang	Southeast University
	Chong Wang	Amazon
	Chuan-Ju Wang	Academia Sinica
	Chunyang Wang	Shanghai Jiao Tong University
	Connie Wang	Beihang University
	Hao Wang	University of Science and Technology of China
	Hongzhi Wang	Harbin Institute of Technology
	Kai Wang	University of New South Wales
	Lebo Wang	Pinterest
	Lijing Wang	New Jersey Institute of Technology
	Limei Wang	Texas A&M University
	Meng Wang	Tongji University
	Qifan Wang	Meta AI
	Sen Wang	School of Information Technology and Electrical Engineering
	Shuwen Wang	Florida Atlantic University, USA
	Sibo Wang	The Chinese University of Hong Kong
	Siyu Wang	The University of New South Wales
	Weiqing Wang	Monash University
	Wentao Wang	Michigan State University
	Xiaojie Wang	Amazon.com, Inc.
	Xiaoyang Wang	University of New South Wales
	Xiaxia Wang	University of Oxford
	Xing Wang	University of Electronic Science and Technology of China
	Xiuling Wang	stevens institute of technology
	Xun Wang	Microsoft
	Yanan Wang	University of Arizona
	Yanhao Wang	East China Normal University
	Yifei Wang	University of California, Berkeley / Meta Platforms Inc.
	Yiwei Wang	National University of Singapore
	Zhenduo Wang	University of Utah
	Zheng Wang	Huawei Singapore Research Center
	Zijie J. Wang	Georgia Tech
	Janus Wawrzinek	Technische Universität Braunschweig
	Michele Weigle	Old Dominion University
	Haokun Wen	Harbin Institute of Technology (Shenzhen)
	Tim Weninger	University of Notre Dame
	Ryen White	Microsoft
	Dawid Wiśniewski	Poznan University of Technology
	Christa Womser-Hacker	University of Hildesheim
	Raymond Chi-Wing Wong	The Hong Kong University of Science and Technology
	Simon Woo	Sungkyunkwan University
	Chenwang Wu	University of Science and Technology of China
	Di Wu	College of Computer and Information Science, Southwest University
	Fangzhao Wu	MSRA
	Han Wu	Anhui Province Key Lab. of Big Data Analysis and Application, University of S&T of China
	I-Chin Wu	National Taiwan Normal University
	Jiancan Wu	University of Science and Technology of China
	Jun Wu	University of Illinois at Urbana-Champaign
	Kun Wu	Stevens Institute of Technology
	Lianlong Wu	University of Cambridge
	Likang Wu	University of Science and Technology of China
	Man Wu	Florida Atlantic University
	Muchen Wu	LinkedIn
	Shengli Wu	University of Ulster
	Wentao Wu	Microsoft Research
	Yongkai Wu	Clemson University
	Youxi Wu	Hebei University of Technology
	Ziwei Wu	University of Illinois at Urbana-Champaign
	Meng Xiao	CAS
	Ding Xiaoou	Harbin Institute of Technology
	Xin Xin	Shandong University
	Bo Xiong	University of Stuttgart
	Feiyu Xiong	Alibaba Group
	Bo Xu	Dalian University of Technology
	Cai Xu	Xidian University
	Depeng Xu	University of North Carolina at Charlotte
	Hongyan Xu	Tianjin University
	Hua Xu	Tsinghua University
	Jianqiu Xu	Nanjing University of Aeronautics and Astronautics
	Jun Xu	Renmin University of China
	Kevin S. Xu	Case Western Reserve University
	Shuai Xu	Nanjing University of Aeronautics and Astronautics
	Shuyuan Xu	Rutgers University
	Xovee Xu	University of Electronic Science and Technology of China
	Yuanbo Xu	jilin university
	Zhe Xu	University of Illinois at Urbana-Champaign
	Niannan Xue	Yelp
	Shan Xue	Macquarie University
	Takeshi Yamada	Faculty of Informatics, Kindai University
	Huan Yan	Tsinghua University
	Rui Yan	Renmin University of China
	Carl Yang	Emory University
	Eugene Yang	Human Language Technology Center of Excellence, Johns Hopkins University
	Kai Yang	Yangzhou University
	Kai-Cheng Yang	Indiana Universiy
	Linglin Yang	Peking University
	Ning Yang	Sichuan University
	Sean Bin Yang	Aalborg University
	Shiyu Yang	Guangzhou University
	Shuiqiao Yang	University of Technology Sydney
	Tao Yang	University of Utah
	Xu Yang	Shandong University
	Yonghui Yang	Hefei University of Technology
	Zhou Yang	The George Washington University
	Yuan Yao	Nanjing University
	Zesheng Ye	University of Melbourne
	An-Zi Yen	National Yang Ming Chiao Tung University
	Xiuwen Yi	JD Intelligent Cities Research
	Wangyang Ying	Arizona State University
	Fan Yixing	ict
	Di You	Worcester Polytechnic Institute
	Jifan Yu	Keg of Tsinghua University
	Philip Yu	University of Illinois Chicago
	Puxuan Yu	University of Massachusetts Amherst
	Yanwei Yu	Ocean University of China
	Zhengtao Yu	Kunming University of Science and Technology
	Long Yuan	Nanjing University of Science and Technology
	Linan Yue	University Of Science And Technology Of China
	Tianzi Zang	Shanghai Jiao Tong University
	Eva Zangerle	University of Innsbruck
	Yuxiang Zeng	The Hong Kong University of Science and Technology
	Chen Jason Zhang	Hong Kong Polytechnic University
	Chengzhi Zhang	Nanjing University of Science and Technology
	Dalin Zhang	Department of Computer Science, Aalborg University
	Danqing Zhang	Amazon
	Fan Zhang	Guangzhou University
	Hainan Zhang	Beijing University of Aeronautics and Astronautics
	Hengtong Zhang	SUNY at Buffalo
	Jianguo Zhang	Salesforce Research
	Jilian Zhang	Jinan University, Guangzhou China
	Ke Zhang	Dataminr, inc
	Le Zhang	Baidu Research
	Lei Zhang	LinkedIn
	Min Zhang	Tsinghua University
	Ningyu Zhang	Zhejiang University
	Ruqing Zhang	CAS Key Lab of Network Data Science and Technology, Institute of Computing Technology, Chinese Academy of Sciences
	Shijie Zhang	The University of Queensland
	Wenjie Zhang	The University of New South Wales
	Xuanyu Zhang	Du Xiaoman
	Xuyun Zhang	Macquarie University
	Yang Zhang	university of science and technology of china
	Yinan Zhang	Nanyang Technological University
	Yipeng Zhang	CSIRO
	Zeyu Zhang	Huazhong Agricultural University
	Zheng Zhang	School of ITEE, The University of Queensland
	Zixuan Zhang	Shanghai Jiao Tong University
	Hongke Zhao	Tianjin University
	Pengpeng Zhao	soochow university
	Wayne Xin Zhao	Renmin University of China, School of Information
	Xiang Zhao	National University of Defense Technology
	Xiangyu Zhao	City University of Hong Kong
	Ying Zhao	Tsinghua University
	Jianming Zheng	National University of Defense Technology
	Min Zheng	Stevens Institute of Technology
	Yong Zheng	Illinois Institute of Technology
	Baifan Zhou	OsloMet
	Dawei Zhou	Virginia Tech
	Fan Zhou	School of Information and Software Engineering, University of Electronic Science and Technology of China
	Kaixiong Zhou	Rice University
	Rui Zhou	Swinburne University of Technology, Australia
	Yi Zhou	University of Electronic Science and Technology of China
	Guanghui Zhu	Nanjing University
	Peide Zhu	Delft University of Technology
	Xiaofeng Zhu	Massey University
	Xingquan Zhu	Florida Atlantic University
	Yanmin Zhu	Shanghai Jiao Tong University
	Yaochen Zhu	University of Virginia
	Yuanyuan Zhu	Wuhan University
	Ziwei Zhu	George Mason University
	Jun Zhuang	Boise State University
	Yong Zhuang	Grand Valley State University
	Matteo Zignani	Università degli Studi di Milano
	Morteza Zihayat	Toronto Metropolitan University
	Imed Zitouni	Google
	Lixin Zou	Wuhan University
	Jingwei Zuo	Technology Innovation Institute
